Accessible computational materials design with high fidelity and high throughput

Despite multiple successful applications of high-throughput computational materials design from first principles, there is a number of factors that inhibit its future adoption. Of particular importance are limited ability to provide high fidelity in a reliable manner and limited accessibility to non-expert users. We present example applications of a novel approach, where high-fidelity first-principles simulation techniques, Density Functional Theory with Hybrid Screened Exchange (HSE) and GW approximation, are standardized and made available online in an accessible and repeatable setting. We apply this approach to extract electronic band gaps and band structures for a diverse set of 71 materials ranging from pure elements to III-V and II-VI compounds, ternary oxides and alloys. We find that for HSE and G0W0, the average relative error fits within 20%, whereas for conventional Generalized Gradient Approximation the error is 55%. For HSE we find the average calculation time on an up-to-date server centrally available from a public cloud provider to fit within 48 hours. This work provides a cost-effective, accessible and repeatable practical recipe for performing high-fidelity first-principles calculations of electronic materials in a high-throughput manner.

==> _guidelines/source.tex <==
% ****************************************************** %
%               NOTES
% ****************************************************** %
Pay attention to formatting - keep spaces, tabs, newlines for clarity.

% ****************************************************** %
%               EXAMPLE TABLE
% ****************************************************** %
\begin{table}
    \caption{
        Caption ....
    }
    \label{table:Hardware}
    \begin{tabular}{l l cccc}
        Provider & Nodes & Cores & Freq. & RAM & Net\\
        \hline
        AWS-*       & c4.8xlarage       & 18 & 2.9 & 60  & 10 \\
        Azure-AZ    & Standard\_F16s    & 16 & 2.4 & 32  & 10 \\
        Azure-IB-A  & A9                & 16 & 2.6 & 112 & 32 \\
        Azure-IB-H  & H16               & 16 & 3.2 & 112 & 54 \\
        SoftLayer   & Virtual           & 16 & 2.0 & 64  & 1 \\
        Rackspace   & Compute1-60       & 16 & 2.8 & 60  & 5 \\
        NERSC       & Edison            & 24 & 2.4 & 64  & 64
    \end{tabular}
\end{table}

% ****************************************************** %
%               EXAMPLE FIGURE
% ****************************************************** %
\begin{figure}[ht!]
    \label{fig-1}
    \includegraphics[width = 0.48\textwidth]{Fig-1.eps}
    \caption{
        Caption...
    }
\end{figure}
